Unique inclusions of maximal C-clones in maximal clones

$\mathit{C}$-clones are polymorphism sets of so-called clausal relations, a special type of relations on a finite domain, which first appeared in connection with constraint satisfaction problems in [Creignou et al. 2008]. We completely describe the relationship w.r.t. set inclusion between maximal $\mathit{C}$-clones and maximal clones. As a main result we obtain that for every maximal $\mathit{C}$-clone there exists exactly one maximal clone in which it is contained. A precise description of this unique maximal clone, as well as a corresponding completeness criterion for $\mathit{C}$-clones is given.

==> hyphexcept.tex <==
%
%
%
\hyphenation{an-aly-ses}
\hyphenation{an-aly-sis}
\hyphenation{as-so-cia-tive}
\hyphenation{as-so-cia-tiv-ity}
\hyphenation{auto-morph-ic}%
%
%
\hyphenation{au-tono-mous}
\hyphenation{au-tono-mous-ly}%
\hyphenation{be-tween}
\hyphenation{Bool-ean}
\hyphenation{bound-ed}%
\hyphenation{Car-te-sian}
%
%
\hyphenation{com-mu-ta-tive}
\hyphenation{com-mu-ta-tiv-ity}
\hyphenation{con-se-quence}
\hyphenation{con-se-quences}
\hyphenation{Con-se-quent-ly}%
\hyphenation{con-se-quent-ly}%
\hyphenation{co-ord-in-ate}
\hyphenation{Def-in-ition}
\hyphenation{def-in-ition}
\hyphenation{Def-in-itions}
\hyphenation{def-in-itions}
\hyphenation{de-ter-mine}
\hyphenation{de-ter-mined}
\hyphenation{de-ter-mined-ly}%
\hyphenation{de-ter-min-ing}
\hyphenation{endo-morph-ic}%
\hyphenation{endo-morph-ism}
\hyphenation{endo-morph-isms}
\hyphenation{equiva-lence}
\hyphenation{equiva-lences}
\hyphenation{equiva-lent}
\hyphenation{equiva-lent-ly}%
\hyphenation{idem-po-tent}%
\hyphenation{idem-po-tents}
\hyphenation{iden-ti-cal}
\hyphenation{Im-pli-ca-tion}
\hyphenation{im-pli-ca-tion}
\hyphenation{Im-pli-ca-tions}
\hyphenation{im-pli-ca-tions}
\hyphenation{ir-re-du-ci-bil-ity}
%
%
%
%
\hyphenation{iso-morph-ic} %
%
%
\hyphenation{lem-ma}%
\hyphenation{Lem-ma}%
\hyphenation{More-over}
\hyphenation{more-over}
\hyphenation{neigh-bour-hood}
\hyphenation{neigh-bour-hoods}
\hyphenation{non-au-tono-mous}
\hyphenation{poly-morph-ic}%
%
%
\hyphenation{posi-tive-ly}%
\hyphenation{prod-uct}
\hyphenation{prod-ucts}
\hyphenation{re-la-tion-al}%
\hyphenation{re-la-tion-al-ly}%
\hyphenation{semi-group}
\hyphenation{semi-groups}
\hyphenation{semi-lat-tice}
\hyphenation{semi-lat-tices}
\hyphenation{strength-en}%
\hyphenation{strength-ened}
\hyphenation{tauto-logic-al}%
\hyphenation{tauto-logic-al-ly}%
\hyphenation{tau-tolo-gies}
\hyphenation{tau-tolo-gous}
\hyphenation{tau-tol-ogy}
\hyphenation{topo-logic-al}%
\hyphenation{topo-logic-al-ly}%
\hyphenation{Top-olo-gies}
\hyphenation{top-olo-gies}
\hyphenation{Top-ology}
\hyphenation{top-ology}

